TRUST: Triangle Counting Reloaded on GPUs

Triangle counting is a building block for a wide range of graph applications. Traditional wisdom suggests that i) hashing is not suitable for triangle counting, ii) edge-centric triangle counting beats vertex-centric design, and iii) communication-free and workload balanced graph partitioning is a grand challenge for triangle counting. On the contrary, we advocate that i) hashing can help the key operations for scalable triangle counting on Graphics Processing Units (GPUs), i.e., list intersection and graph partitioning, ii)vertex-centric design reduces both hash table construction cost and memory consumption, which is limited on GPUs. In addition, iii) we exploit graph and workload collaborative, and hashing-based 2D partitioning to scale vertex-centric triangle counting over 1,000 GPUswith sustained scalability. In this work, we present TRUST which performs triangle counting with the hash operation and vertex-centric mechanism at the core. To the best of our knowledge, TRUSTis the first work that achieves over one trillion Traversed Edges Per Second (TEPS) rate for triangle counting.

==> background.tex <==
\section{Background}
\label{sec:background}

\subsection{Notation and Terminology}

% Various notations used in the paper for the graph are listed in the table~\ref{Table:notation}.
% \vspace{-1cm}
% \begin{table}[t]

% 	\centering

% 	\begin{tabular}{ll}
% 		\hline
% 		\textbf{Terminology}    & \textbf{Description} \\ \hline
% 		$G (V, E)$ & Graph with vertex and edge sets as V and E   \\ \hline
% % 		Adjacency matrix                & $A$        \\ \hline
% % 		Edge tuple representation     & $(u, v)$    \\ \hline
% % 		Triangle     			& $(u, v, w)$    \\ \hline
% 		$d(u)$    & Out degree of a vertex $u$ \\ \hline
% 		$N(u)$ &Out neighbor lists of a vertex $u$     \\ \hline
% 		$H_u$&Hash table of $N(u)$     \\ \hline
% 		$\Delta_{u, v, w}$ & A triangle formulated by vertices $u, v$ and $w$\\ \hline
% 		$BN$ & bucket number in hash table
% 		% CSR (G) & The Compressed Sparse Row (CSR) format of graph G
% 		\\ \hline

% 	\end{tabular}
% 	\caption{The notations used through this paper.\vspace{-0.2in}}
% 	\label{Table:notation}
% \end{table}



% Table~\ref{Table:notation} presents various terminologies and notations that are used through this paper. 
Let $G (V, E)$ be an undirected and unweighted graph, $V$ and $E$ are the vertex set and edge set of $G$, respectively. 
In spite of a great visualization tool~\cite{maaten2008visualizing}, \textit{a graph cannot be stored in the way we see it}. Often graphs are stored in array style data structures, among which edge list and Compressed Sparse Row (CSR) are the mainstream options.
Particularly, the edge list is a collection of all the edge tuples in $G$, where each tuple $(u, v)$ is an edge from $u$ to $v$ in $G$. CSR is the compressed format of the adjacency matrix, which stores the neighbors of each vertex in a row. It uses two arrays, i.e., begin position and adjacency list.
The adjacency list is a concatenation of the out neighbor lists of all vertices in the graph, and the begin position specifies the starting position of the neighbor list of each vertex.

% In begin position, the index represents the vertex ID and the value stored in the array represents the starting index of neighbors of the vertex in the adjacency list. In \hash, we only need CSR graph format in memory.
\vspace{-0.1in}
\subsection{Triangle Counting {Algorithms}}

This section describes the mainstream triangle counting algorithms, i.e., intersection, and other alternatives - matrix-multiplication and subgraph-matching based methods. \update{Table~\ref{tab:related} categorizes these closely related projects.}



% There mainly exist three types of triangle counting algorithms, that is, intersection, subgraph matching and matrix multiplication based approaches. 

 

% Since undirected graph might count a triangle six times, graph orientation which reduces the edge by half is often performed before counting triangles.
% Mainstream triangle counting algorithms mainly consists of efforts in two directions, graph computing and mining. 
% \vspace{0.1in}

\textbf{Intersection based approach} encompasses three algorithm options, i.e., merge-path, binary-search, and hashing, which could be implemented in vertex-centric or edge-centric fashion.  
%\lld{The reasoning doesn't make sense to me.}
%\fixme{Moved to Intro}
%\lld{This paragraph could be in intro when vertex- and edge-centric are first mentioned. Or try to be more vague when describe them in intro. It's hard to understand them in intro.}
\textit{Merge-path based intersection}, as shown in Figure~\ref{intersection}(b) uses two pointers to scan through two lists from beginning to end in order to find the intersection between them. During scanning, the pointer that points to a smaller value will be increased. A triangle is enumerated if both pointers need to be increased (i.e., they point to the same vertex). \update{\cite{shun2015multicore,giechaskiel2015pdtl,hu2016efficient} observe that merge-path suits CPU based triangle counting due to lower time complexity compared with binary-search and higher cache hit rate compared with hashing.}
\textit{Binary-search based intersection} organizes the longer list as a binary tree and uses the shorter list as search keys. For each search key, it descends through the binary-search tree in order to find the equal entries, which is a triangle. \update{Hu et al.~\cite{hu2018tricore,hu2017trix,hu2018high} indicate that edge-centric binary-search fits GPU based triangle counting because of higher parallelism and more balanced workloads.}
\textit{Hashing based intersection} constructs a hash table for one list, then uses the other list as search keys to find the common elements in the hash table. Particularly,~\cite{shun2015multicore} only allows one element in each hash bucket of the hash table, which is also referred to as open addressing. When collision surfaces, this method uses linear probing to manage the element, as well as to search for common elements during intersection. {To avoid high cost on linear probing, this method ends up with large hash tables.} 
% \cite{shun2015multicore} first construct hash table for each vertex's neighbor list, so they require more memory to store these hash tables. While~\cite{pandey2019h} dynamic constructs the hash table for one list to save the memory of hash table.\confuse{do we need to discuss H-INDEX method here? They are different}. So~\cite{shun2015multicore} always use smaller list as searching key. They only allow one element at each bucket in hash table (which is also called open addressing). When they're facing collision, they will use linear probing to find a next empty bucket and put the new element into that bucket. So they require large bucket number to avoid collision which lead to lower cache hit.\confuse{updated, please take a look}
% \confuse{Here we only show the intersection of M and N, and reader may think they dynamic construct the hash table, but shun's paper construct hash table in the preprocessing so they require more memory. Further they use open addressing (Linear probing) manage collision we use separate chaining manage collision.} 
% \confuse{it's not this papers method, they don't have collision} uses hash to divide the two lists into buckets. Inside of each bucket pair, one can use linear search, binary search or merge path to find the common entries which is a triangle.
\textit{Bitmap}
% ~\cite{bisson2017high,bisson2018update,che2019accelerating}
can be thought of as a hash table with $|V|$ {buckets}, which eliminates collision but consumes significantly more memory. \update{Bisson et al.~\cite{bisson2018update,bisson2017static,bisson2017high} perform vertex-centric GPU-based triangle counting. However, these projects use bitmap to implement hash tables, which suffers from high memory consumption and is hence only suitable for small graphs. Some external triangle counting projects~\cite{hu2013massive,hu2014efficient} also explore the bitmap option since they have large external storage. }
% . And there has no collision in bucket and compression method can be deployed to save memory. However, it needs much more memory than other method. 
% On another level, bitmap can be thought as a line in adjacent matrix, $bitmap_u(w)=1$ means $w$ is neighbor of $u$.


% to find out  assume $N(u)$ has been sorted, each element in $N(v)$ uses binary-search to determine whether it is in $N(u)$. 

Figure~\ref{intersection} explains how the aforementioned three intersection algorithms work on two lists M and N. As shown in Figure~\ref{intersection}(b), merge-path will use the vertical and horizontal pointers to scan through these two lists. Since the first element in M, i.e., 2, is smaller than that of N, the vertical pointer will be increased. Further, because both M and N have 3 as their elements, both pointers will be increased, and one triangle is enumerated. Similarly, we can enumerate all the triangles. In binary-search based method, as shown in Figure~\ref{intersection}(c), we will use each element of M as the search key to search against the binary tree of N. For element 3 of M, the search keeps descend on the left side of N in order to find the triangle. 
% \confuse{do we need use $M$ or other}
% \fixme{Hash-based intersection divides both neighbor lists into four buckets. And inside of each bucket pair, using the first pair as an example, we need to figure out whether \{4\} is equal to any entry in \{4, 8\} bucket.}
% Hash-based intersection first construct hash table for each neighbor list in a graph. When intersection two lists, it will search the elements of smaller list in larger list's hash table. 
% \fixme{Explain Figure 1(d)}\confuse{added}
Figure~\ref{intersection}(d) depicts the hashing based solution in~\cite{shun2015multicore}. This method first constructs a hash table for longer list N. Since $\textsc{hash}(8)=\textsc{hash}(18)$, element 18 will use linear probing search 8 and the elements after 8 in order to find the common element. 
% the next bucket 9 (blue one). After hash table has been constructed, the search key in $M$ will search the hash table for the common element. 
% \fixme{What if we have 18 in M? when will we stop? We will stop until the empty bucket or find the element}


{Some intersection based approaches often exploit the graph orientation technique to reduce the number of edges present in the graph by half for avoiding redundant work~\cite{shun2015multicore,pearce2017triangle}. 
% \update{~\cite{shun2015multicore}}.
For a pair of undirected edges, \textit{rank-by-degree} technique removes the edge whose source degree is larger than the destination degree and preserves the remaining edge. With the orientation technique, we achieve lower triangle counting time.} 
% each element in list M will be searched in hash table of N. For the element 3 in M it will search bucket 3. To see more detail of parallel insert elements into hash table with open addressing, you can read~\cite{shun2014phase}.\confuse{do we need mention this}

% \fixme{related work does hash for both lists}
% \confuse{In this section, we say we divide two lists, but in real we only need to partition one list.}

% Intersection-based approach also exploits graph orientation reduces the edge by half before counting trianlges in order to avoid counting identical triangles by six times.
% For a pair of undirected edges, rank-by-degree deletes the edge whose source degree is larger than the destination and preserves the other. Doing this, we achieve two goals, that is, correctness and lower time complexity. First, randomly removing one direction of the undirected edge does not ensure correctness for triangle counting. Fixing the order of deletion can both remove duplicate edges and ensure we do not miss any triangle. 

% this approach ensures minimize the time complexity for intersection-based design~\cite{}

% $(u, v)$ is stored by $u$ as out-going edge if $d(u)<d(v)$, or $u<v$ when $d(u) = d(v)$.

% triangle (2,3,4) will be counting 6 times as (2,3,4), (2,4,3), (3,2,4), (3,4,2), (4,2,3), (4,3,2). To avoiding useless work and reducing the time complexity, we orientate each edge from undirected to directed. For graph orientation, we implement $rank-by-degree$ as in~\cite{shun2015multicore}.  As randomly removing one direction of the undirected edge does not ensure correctness for triangle counting, a fix order is used to remove duplicate edges to ensure we do not miss any triangle. This orientation also improves the performance of triangle counting as it reduces the variance of degree distribution in the graph. Fig~\ref{fig:graph}(b) shows the directed graph after $rank-by-degree$ orientation for graph~\ref{fig:graph}(a). In section \ref{sec:preprocessing}, we discuss orientation in detail.
 
% This section describes the mainstream triangle counting algorithms, i.e., intersection, and other alternatives, such as matrix multiplication and subgraph matching based methods. 

%  \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{fig/matrix_triangle.pdf}
%     \caption{Matrix multiplication based triangle counting.\vspace{-.15in}}
%     % \fixme{Figure (c) is wrong? also this figure is too small}\confuse 
%     % choose which image(in ppt)}
% 	\label{fig:matrix_tc}
% % 	\vspace{-0.6cm}
% \end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/matrix_mul.pdf}
    \vspace{-0.05in}
    \caption{Matrix-multiplication based triangle counting where $\mathrm{A}$ is the adjacency matrix of the graph.
    %\lld{shared memory looks like shared among SMs in this fig.}
    \vspace{-.1in}
    }
	\label{fig:matrix_mul}
\end{figure}


% \vspace{0.05in}
% Figure~\ref{fig:matrix_tc} presents the 
\textbf{Matrix-multiplication based approach}
% ~\cite{azad2015parallel,yacsar2018fast,yacsar2019linear,wolf2017fast,Low2017FirstLL,yasar2019linear,acer2019scalable}
decomposes the adjacency matrix (i.e., A)
% \confuse{we don't describe what is adjacent matrix before} 
of the graph into lower and upper triangular matrices $\mathrm{L}$ and $\mathrm{U}$, respectively, as shown in Figure~\ref{fig:matrix_mul}.
% $\mathrm{L}$ contains the edges where source $>$ destination, and $\mathrm{U}$ otherwise.
Let $\mathrm{B} = \mathrm{L}\cdot \mathrm{U}$. This multiplication actually counts the number of wedges, also referred to as open triangle, with $u\rightarrow v$ and $v\rightarrow w$. 
% \lld{explain wedge?}
% lges $(u, v, w)$. $B_{uw}$ means the number of $v$ that have edges $(v,u)$ and $(v,w)$ while $v<u$ and $v<w$. 
% The decomposition of matrix $\mathrm{A}$ is a kind orientation that orientate by vertex ID. Assume the adjacent matrix after orientation is $\mathrm{O}$, we can also compute $\mathrm{B}=\mathrm{O}*\mathrm{O}^{\mathrm{T}}$. 
The further element-wise multiplication (i.e., Hadamard Product) of $\mathrm{A}$ and $\mathrm{B}$ determines whether the wedge is closed.%$A[u][w]$. 
 Finally, 
we summarize the number of non-zero elements in the resultant matrix. 
% gives the count of triangles in the graph. 
Since each edge is counted by both vertices, the final sum is divided by 2 to get the exact count of triangles. Using Figure~\ref{fig:matrix_mul} as an example, because the $\mathrm{L}[2][] = [1, 0, 0, 0]$ and multiply the $\mathrm{U}[][3] = [1, 0, 1, 0]$ will arrive at 1 at $\mathrm{B}[2][3] = 1$, it means there is a wedge between $(2, 0)$ and $(0, 3)$. Afterwards, element-wise product between $\mathrm{A}[2][3]$ and $\mathrm{B}[2][3]$ can confirm whether there is an edge which closes the wedge.
\update{It is worth to mention that Yacsar et al.~\cite{yacsar2018fast,yacsar2019linear,wolf2017fast,yasar2019linear,acer2019scalable} leverage KokkosKernels~\cite{KokkosKernels}, a linear algebra library, to count triangles.}
% the exact count is $\frac{4}{2}$= 2. Or we can just calculate the lower triangular matrix of $\mathrm{R}$. Furthermore, techniques like masked matrix multiplication and 1D decomposition can be used to speedup the performance in distributed systems~\cite{7284394}. 

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=.5\linewidth]{fig/tc_SM.pdf}
%     \caption{An example of triangle counting using subgraph matching algorithm for the sample graph in Figure~\ref{fig:graph}.}
%     \label{fig:sm}
% \end{figure}

% \subsection{Subgraph Matching Based Method}
\vspace{0.1in}
\textbf{Subgraph-matching based approach}
% \update{~\cite{wang2016comparative}}
% ~\cite{wang2016comparative,bi2016efficient,lai2015scalable} 
searches for all occurrences of a query graph in a data graph. Triangle counting regards triangle as that query graph.~\cite{wang2016comparative} implements a two-step subgraph matching approach for counting the number of triangles on undirected labeled graphs. First, the query graph - triangle in this case - is factored into a tree and non-tree edges. 
Afterward, one will find all the vertices from the data graph that matches the root of the query tree using degree-based filtering. Subsequently, one will traverse the query tree as well as the data graph from the candidates of the root with the matching rule. Finally, one joins the tree candidates and non-tree edge candidates to arrive at all the isomorphic triangles present in the data graph. 


\subsection{Approximate Triangle Counting}
{Since triangle counting in extremely large graphs is computationally expensive, some researchers also explore approximate triangle counting algorithms to reduce the runtime~\cite{tsourakakis2009doulion,pagh2012colorful,shun2015multicore,arifuzzaman2013patric,wang2019rept,wang2017approximately,rahman2013approximate,mawhirter2018approxg,wu2016counting,avron2010counting,tsourakakis2011spectral,tsourakakis2011counting}.
\cite{tsourakakis2009doulion,rahman2013approximate}
% \update{\cite{rahman2013approximate}}
are based on edge-centric paradigm. They estimate the number of triangles by sampling the edges and counting a fraction of edges' triangle.
\cite{pagh2012colorful,shun2015multicore}
% \update{\cite{shun2015multicore}}
are based on vertex-centric triangle counting. Differing from~\cite{tsourakakis2009doulion,rahman2013approximate}
% \update{~\cite{rahman2013approximate}}
which samples the edges, they sample the vertices. They first color the vertices, then keep the edges that connect two same-colored vertices. Further, they count the triangles in the sampled subgraph and estimate the total triangles present in the graph. \cite{seshadhri2013triadic} approximates the triangle counting by wedge sampling. \cite{wu2016counting} performs a detailed experiment and analytical that compares these different sampling approaches. In addition to graph sampling-based approximate triangle counting, 
% \update{\cite{tsourakakis2011counting}} 
\cite{avron2010counting,tsourakakis2011spectral,tsourakakis2011counting} approximate triangle counting based on spectral decomposition of the graph.} 
%It will be interesting to combine our work with approximation methods to achieve better performance and which we leave as our future work.

\subsection{Graph Partitioning Methods}
\label{sec: related of partition}

Value-range based partitioning, such as 2D partitioning~\cite{bulucc2011parallel}, is one of the most popular approache for triangle counting. In this direction, 
Suri et al.~\cite{suri2011counting} and Park et al.~\cite{park2013efficient} 
% \update{\cite{park2013efficient}}
design a 2D graph partition method based on MapReduce, but suffer from workload imbalance. 
\cite{hu2017trix,hu2018tricore}
% \update{\cite{hu2018tricore}} 
balance the workload of 2D partition on edge-centric triangle counting by a runtime workload stealing scheme. However, this introduces a nontrivial overhead. 
\cite{yacsar2019linear}
% \update{\cite{yacsar2019linear}} 
deploys 2D partition on matrix based triangle counting. Whereas, the workload imbalance problem still exists.
\cite{elenberg2015beyond,hoang2019disttc} 
% \update{\cite{elenberg2015beyond}} 
distribute edges of graph among different machines and cache the vertices requiring communication among the machines during triangle counting. 
\update{METIS~\cite{karypis1998fast} is a well-known topology-aware graph partitioning approach that aims to make balanced vertex/edge yet with lower edge cuts. This method, however, would require inter-worker communication when counting triangles.
% Tricore~\cite{hu2018tricore} simply applies CSR partitioning to scale triangle counting but suffers from workload imbalance. 
%Tricore does not make workloads balance among each task equal. 
% It introduces work-stealing and partition streaming to balance the workload among GPUs leading to additional costs. While scaling to large numbers of GPUs (e.g., 1024), the additional costs will have a significant impact on the total time. 
Recently, LiteTe~\cite{zhang2019litete} also attempts to use value-range based 2D partitioning for triangle counting, but, again, experiences workload imbalance.
}


\subsection{Platforms for Counting Triangles}
{Except using only a CPU or GPU to count triangles, a hybrid system like \cite{yasar2019linear} utilizes both CPU and GPU to speed up triangle counting. \cite{liu2018griffin} schedules the intersection processing to both CPU and GPU. \cite{huang2018triangle} deploys triangle counting in FPGA, which has better energy efficiency. %We leave it as future work to implement {\hash} in a heterogeneous environment.
}

\subsection{Graph Dataset}

\begin{table}[htbp]
    \renewcommand\arraystretch{1.2}
    \centering
    \scalebox{0.89}{
    % \begin{spacing}{2.0}
    \begin{tabular}{|c|c|r|r|r|}
        \hline
        \textbf{Dataset} & \textbf{Abbr.} & \multicolumn{1}{|c|}{\textbf{$|V|$}} & \multicolumn{1}{|c|}{\textbf{$|E|$}}  & \multicolumn{1}{|c|}{\textbf{\# triangles}} \\ \hline
        3Dgrid & 3D    & 99,897,344  & 299,692,032  & 0  \\
        random & RA    & 100,000,000  & 999,999,892  & 1,221  \\ 
        rMat & RM    & 129,594,758  & 996,771,953  & 4,114,616  \\\hline
        Cit-Patents & CP    & 3,774,768  & 16,518,947  & 7,515,023  \\
        Friendster & FS    & 65,608,366  & 1,806,067,135  & 4,173,724,142  \\  
        gsh-2015-host & GH    & 68,660,142  & 1,502,666,069  & 520,901,310,734  \\ 
        it-2004 & IT    & 41,290,682  & 1,027,474,947  & 48,374,551,054  \\
        MAWI & MA   & 128,568,730  & 135,117,420  & 10  \\ 
        Orkut & OR    & 3,072,441  & 117,185,083  & 627,584,181  \\
        Twitter & TW    & 41,652,230  & 1,202,513,046  & 34,824,916,864  \\
        Wikipedia & WK    & 12,150,976  & 288,257,813  & 11,686,212,734  \\ \hline

        % gsh-2015 & GS & 988,490,691&	25,690,705,118	& 910,140,734,636\\
        clueweb12 & CW &955,207,488 &37,372,179,311&1,995,295,290,765 \\
        uk-2014 & UK & 787,801,471 &	42,464,215,550 &	7,872,561,225,874 \\ \hline
    \end{tabular}%
    % \end{spacing}
    }
    \vspace{.05in}
    \caption{Graph datasets.}
    \label{tab:graph dataset}%
    % \vspace{-0.4cm}
\end{table}%

  
Table~\ref{tab:graph dataset} exhibits all the graphs we used to evaluate {\hash}. Broadly, these datasets fall into three types, that is,  synthetic, regular, and large real-world graphs. Particularly, RA, RM, and 3D are generated by the Problem Based Benchmark Suite (PBBS)~\cite{shun2012brief}.
In the regular graph category, MA (Measurement and Analysis on the WIDE Internet) is the Internet traffic archive~\cite{mawi2012mawi}. CP, OR, and FS are from Stanford Network Analysis Project (SNAP) datasets~\cite{leskovec2016snap}. 
TW~\cite{kwak2010twitter} is the Twitter graph, and WK~\cite{konect:2017:wikipedia_link_en} is the English Wikipedia link graph.
% , MAWI dataset from MAWI  (Measurement and Analysis on the WIDE Internet) Working Group traffic archive~\cite{mawi2012mawi}. 
The remaining are web graphs, i.e., IT and GH, as well as the extremely large real-world graphs, i.e., CW and UK from WebGraph~\cite{BoVWFI,BRSLLP,BMSB}. During the evaluation, we transform the graph by following steps: 1) Deleting the duplicate edges and self-loops. 2) Transforming directed graphs to undirected graphs. 3) Removing orphan vertices. The size and number of triangles of these graphs are also included in Table~\ref{tab:graph dataset}. 



% performed to remove the edges that do not contribute to forming a triangle. Second, the joining step collects candidate edges to form a triangle. Figure~\ref{fig:sm} illustrates how subgraph matching techniques can be used for triangle counting. We use the same graph in Figure~\ref{fig:graph}. The graph is filtered to remove the candidate vertices having degree less than 2. Vertex 1 is removed as it's degree is only 1. Also, candidate are labeled based upon boolean candidate set to get the edge list containing only candidate edges. Then, joining step is performed to tests if each combination of edges contribute to a triangle or not. Two triangles with combination of edges $((0, 2), (0, 3), (2, 3))$ and $((4 ,2), (4, 3), (2, 3))$ satisfies the query graph of a triangle. Joining step for this method requires a lot of memory. With an increasing number of edges, the possible edge combination also increases. More details on the implementation can be found at~\cite{wang2016comparative}.

% In graph mining domain, one will first find all open triangles through tree-based prune and subsequently verify whether there exists an edge from the graph that can complete this triangle~\cite{bhattarai2019ceci}. 


% A triangle $\Delta_{u, v, w}$ is formed by three vertices $u, v$ and $w$ that are connected with each other in an undirected graph. 
%  Subsequently, there exist three viable designs to count triangles, that is, \textit{intersection}, \textit{matrix multiplication} and \textit{subgraph matching}. Below, we will briefly discuss orientation and these three viable designs.  


% In Figure~\ref{fig:graph}, vertices (2, 3, 4) and (2, 3, 0) form two different triangles. The time complexity of triangle counting is O$(|E|^{\frac{3}{2}})$. 
%  \td algorithm complexity of TC.


% \subsection{Storing Graph}

% A graph can be stored in the form of edge list, Adjacency matrix or Compressed Sparse Row (CSR). 
% Edge list is a collection of tuples present in a graph represented as $(u, v)$ where $u$ and $v$ are connected with each other. The count of the edge list is equal to the edges present in the graph.
% An adjacency matrix is a matrix representation of the graph with the dimension of $|V| * |V|$. Each position in adjacency matrix $A_{uv}$ = $A_{vu}$ = 1 if and only if there exists an edge between $u$ and $v$.  
% CSR is the compressed format of adjacency matrix which stores the neighbors of each vertex in a row. It uses two arrays: begin position, adjacency list. In begin position, the index represents the vertex ID and the value stored in the array represents the starting index of neighbors of the vertex in the adjacency list. In \hash, we only need CSR graph format in memory.
 

%   \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\linewidth]{fig/graph.pdf}
%     \caption{(a) A sample undirected graph with 6 edges, 5 vertices and 2 triangles. (b) Directed graph after $rank-by-degree$ orientation. }
%     \label{fig:graph}
% \end{figure}


% Thread management, time complexity and memory friendliness. \td


% \section{Background and Related Works}
% \textbf{Graph preprocessing}. 
% We assume $G$ to be an undirected graph for triangle counting. As the graph is undirected, each edge is stored as two directed edges in the graph format. This duplication leads each triangle to be counted multiple time incurring redundant work. For example, triangle (2,3,4) will be counting 6 times as (2,3,4), (2,4,3), (3,2,4), (3,4,2), (4,2,3), (4,3,2). To avoiding useless work and reducing the time complexity, we orientate each edge from undirected to directed. For graph orientation, we implement $rank-by-degree$ as in~\cite{shun2015multicore}. Each edge $(u, v)$ is stored by $u$ as out-going edge if $d(u)<d(v)$, or $u<v$ when $d(u) = d(v)$. As randomly removing one direction of the undirected edge does not ensure correctness for triangle counting, a fix order is used to remove duplicate edges to ensure we do not miss any triangle. This orientation also improves the performance of triangle counting as it reduces the variance of degree distribution in the graph. Fig~\ref{fig:graph}(b) shows the directed graph after $rank-by-degree$ orientation for graph~\ref{fig:graph}(a). In section \ref{sec:preprocessing}, we discuss orientation in detail.



% Furthermore, improve the large degree vertex's locality definitely better than improve small degree vertex in triangle counting problem, while these methods treat them as equal. 


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.8\linewidth]{fig/graph_partition.pdf}
%     \caption{Graph partition of graph in Figure~\ref{fig:graph}. (a) 1-D partition of the adjacency matrix. (b) 2-D partition of the adjacency matrix.}
%     \label{fig:partition}
% \end{figure}
% \begin{figure*}[hbt!]
% 	\centering
% 	\includegraphics[width=.98\textwidth]{./fig/intersection-sa.pdf} 
% %	\includegraphics{./Figures/matrix_graph_etree.pdf} 
% % 	\caption{Sequential implementation of fill-path theorem from~\cite{rose1978algorithmic}.} %caption is the title of image
% 	\caption{Various triangle counting algorithms for the sorted (a) input lists. Particularly, we assume two threads working on the intersection with (b) merge-path based approach, (c) binary-search approach, (d) {\hash} approach with memory friendly bucket storage format.}
% % 	(which is similar to {\hash} assisted binary-search approach and (e) {\hash} assisted merge-path.} %caption is the title of image
% 	\label{fig:tc} %  used for citing
% 	%   \vspace{-.1in}	
% \end{figure*}

% \subsection{Graph Partitioning}
%  Graph partitioning reduces a graph into smaller graphs. The graph is divided into multiple partition based upon memory bound $M$ to fit each partition in the GPU's memory. The partition technique is also used for distributed systems or external memory systems processing large graph for higher level of parallelization and scalability. Figure ~\ref{fig:partition} shows an example how graph partition can be performed in 1-D or 2-D. 1D partition divides the vertex set $V$ into roughly equal $P$ disjoint subsets. For 2-D partition, we first perform a 1-D vertical cut of vertex set. Then, a horizontal cut is performed over each partition to achieve 2-D partition blocks. 2-D partitions is more balanced than 1-D partitions. Memory limit $M$ bounds the size of each partition for both partitioning method.  {\hash} partitions the graph for in-memory multi-GPU implementation of triangle counting.


==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
This paper introduces {\hash} that reloads triangle counting on GPUs. Particularly, it comes with vertex-centric hashing based algorithm, collision and workload balance optimizations, and workload and graph collaborative partitioning techniques. Taken together, {\hash}, to the best of our knowledge, is the first work that advances triangle counting beyond trillion TEPS rate.

\section{Acknowledgement}
\final{
We thank the anonymous reviewers for their helpful suggestions and feedback. This research is supported in part by the National Science Foundation CRII award No. 2000722, the U.S. Department of Energy, Office of Science, Office of Advanced Scientific Computing Research, under Contract No. DE-AC02-05CH11231 at Lawrence Berkeley National Laboratory, and Brookhaven National Laboratory, which is operated and managed for the  U.S. Department of Energy, Office of Science by Brookhaven Science Associates  under contract No. DE-SC0012704, the National Key R\&D Program of China 2018YFB1003505, the National Natural Science Foundation of China under Grant Numbers 61772265, 61802172, 62072228, and 61872176, the Leading-edge Technology Program of Jiangsu Natural Science Foundation (No. BK20202001), and National Key R\&D Program of China under Grant 2020YFB1005900.}



% based approach for triangle counting that avoids the preprocessing step of sorting the neighbor list. For better memory access pattern, we further introduce interleaved format for the hash bucket storage. With up to 16 GPUs, {\hash} achieves $>$ $10^{10}$ TEPS for some graphs. 


==> introduction.tex <==
\IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}
% \td Using double hashing. First find a bin. Then again hash it to find the position within the bin. \td \newline

\noindent
% For a graph of interest, t
The number of triangles (i.e., three-vertex clique) is a key metric to extract insights for a wide range of graph applications, such as, anomaly detection~\cite{noble2003graph,akoglu2015graph},
% \update{~\cite{akoglu2015graph}},
community detection~\cite{prat2014high,prat2016put,zhang2016efficient,rezvani2018efficient},
% \update{~\cite{rezvani2018efficient}},
and robustness analysis~\cite{dekker2004network}. For more thorough studies about the applications surrounding triangle counting, we refer the readers to recent surveys~\cite{schank2007algorithmic,chu2011triangle,al2018triangle}.
% \update{~\cite{al2018triangle}}
%
% \confuse{Is these paper ok?}. 
Further, triangle counting is also a basic primitive for an array of graph algorithms, e.g., clustering coefficient~\cite{watts1998collective}, k-truss~\cite{wang2012truss,date2017collaborative,smith2017truss},
% \update{~\cite{smith2017truss}},
and transitivity ratio~\cite{wasserman1994social}. Ultimately, the significance of triangle counting is pronounced by the GraphChallenge~\cite{graphchallenge} competition, where 
% participating projects from all over the world 
participants
are ranked by how fast they perform triangle counting on a collection of graph datasets.  


% Triangle counting gains popularity from social network analysis, where it is exploited to detect communities and measure the corresponding cohesiveness~\cite{hu2018tricore,wang2016comparative}. Particularly, one can use triangle counting to measure the robustness of the graph - the deletion of an edge in a triangle will not result in disconnection of these three vertices. It is also worthy of noting that triangle counting is a primary routine for local and global clustering coefficient analysis of a network~\cite{schank2004approximating}.


% Attracted by the great impacts of triangle counting, 

% The number of projects centering around triangle counting thus soars! 
% \update{There exists a variety of projects centering around triangle counting.}
\update{Recent years have witnessed a surge of projects in triangle counting.}
Briefly, triangle counting efforts fall into three categories, that is, list intersection, matrix operation, and subgraph matching. 
% to count triangles\confuse{delete to count triangles?}
List intersection further encompasses two system implementation methods, i.e., edge- and vertex- centric options. In terms of how to intersect the lists, one can exploit merge-path, binary-search, and hashing-based algorithms. Note, the bitmap is an extreme case of hashing where the number of buckets equals the number of vertices. All the details about these methods are thoroughly discussed in Section~\ref{sec:background}. 

The efforts of seeking suitable hardware platforms to accelerate triangle counting also gain momentum, popular attempts include multi-core CPUs~\cite{shun2015multicore,pearce2017triangle,elenberg2015beyond,arifuzzaman2015fast},
% \update{~\cite{shun2015multicore}},
many-core GPUs~\cite{hu2018tricore,hu2017trix,hu2018high,hoang2019disttc,pandey2019h}, 
% \update{~\cite{hu2018tricore}},
and external memory devices~\cite{hu2013massive,giechaskiel2015pdtl,cui2018efficient,hu2014efficient,hu2016efficient}.
% \update{~\cite{cui2018efficient}}.
Of all these platforms, GPUs are particularly tempting for the following reasons. 
% \fixme{First, HBM. Second, shared memory. Third, registers. @wzb please add details for each aspect.} 
First and foremost, GPUs come with unprecedented computing and data delivering capabilities. Using recent NVIDIA Tesla V100~\cite{nvidia2017v100} GPU as an example, it provides 80 streaming multiprocessor (SM) and 64 FP32 cores/SM, which can reach 15.7 TFLOPS peak performance. Along with High Bandwidth Memory (HBM2) on device, this GPU can retain 900 GB/s memory bandwidth. 
% Second, 
The massive parallelism and fast memory support are well suited for triangle counting. 
Second, GPUs are equipped with configurable on-chip shared memory where users can store frequently accessed data structures. As we will discuss shortly, shared memory can significantly improve the efficiency of triangle counting.
Last but not least, GPUs feature a hierarchical thread organization, e.g., thread, warp, and Cooperative Thread Array (CTA), which fits graphs that come with inherent workload imbalance across various vertices. 

%  First GPU has fast HBM, that support massive thread load from global memory. Second shared memory is design for thread in a block, they can fast access shared memory. Third, GPU support massive register.

\vspace{-0.05in}
\subsection{Related Work and Challenges}
\label{subsec:pitfall}

Reviewing the recent literatures centering around triangle counting,
% ~\cite{bisson2017static,shun2015multicore,che2019accelerating,bisson2017high,yacsar2018fast,bisson2018update,yacsar2019linear,wolf2017fast,yasar2019linear,hu2017trix,hu2018tricore,hu2018high,hu2019triangle,date2017collaborative,pearce2017triangle,elenberg2015beyond,arifuzzaman2015fast,hu2013massive,hoang2019disttc,pandey2019h,hu2016efficient,giechaskiel2015pdtl,cui2018efficient,zhang2019litete,green2014fast,azad2015parallel,hu2014efficient,Low2017FirstLL,acer2019scalable,wang2016comparative,DBLP:conf/alenex/2014,DBLP:conf/alenex/OrtmannB14,zhang2016efficient,hu2015join,ding2018privacy,lu2017exploring,zhu2017efficient,yu2020aot,chu2011triangle,pearce2013scaling}, 
we arrive at the following challenges faced by vertex-centric hashing-based triangle counting, along with brief discussions about our resolutions.  
% - {edge-centric list intersection is the most popular option for triangle counting}. In terms of intersection algorithms, merge-path excels on CPU while binary-search bests on GPU. When it comes to distributed triangle counting, edge-centric again prevails. We explain the key reasons behind these pitfalls and our resolutions as below: 


% have explored the possibility of applying hashing to aid triangle counting, they fall short at fully unleash the potential of hashing.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[htbp]
	\renewcommand\arraystretch{1}
	\scalebox{0.85}{
	\begin{tabular}{|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{}  & \multirow{2}{*}{\textbf{Binary-search}} & \multirow{2}{*}{\textbf{Merge-path}} & \multirow{2}{*}{\textbf{Bitmap}} & \multicolumn{2}{c|}{\textbf{Hashing}} & \multirow{2}{*}{\textbf{Matrix-multiplication}}  & \multirow{2}{*}{\textbf{Subgraph-matching}} \\ \cline{5-6} 
		&  &  &  &   \textbf{Vertex-centric} & \textbf{Edge-centric} & &\\ \hline
		\textbf{CPU}  & ~\cite{date2017collaborative} (CPU+GPU) & ~\cite{shun2015multicore,giechaskiel2015pdtl,hu2016efficient} & \cite{hu2013massive,hu2014efficient} & ~\cite{shun2015multicore} & & ~\cite{ azad2015parallel, Low2017FirstLL, acer2019scalable,yacsar2018fast,yacsar2019linear,wolf2017fast} & \cite{bi2016efficient,lai2015scalable}\\ \hline
		\textbf{GPU}  & ~\cite{hu2018tricore,hu2017trix,hu2018high,hu2019triangle, hoang2019disttc} & ~\cite{green2014fast} & ~\cite{bisson2018update,bisson2017high,bisson2017static} & \textbf{\hash} & ~\cite{pandey2019h}&  ~\cite{yasar2019linear, wang2016comparative} & \cite{wang2016comparative}\\ \hline
	\end{tabular}
	}
	\caption{\update{Closely related projects for {\hash}.}}
	\label{tab:related}
	\vspace{-0.25in}
\end{table*}

\vspace{0.05in}
\textit{Challenge 1}. 
The hashing-based intersection is not suitable for triangle counting resulting from the concern of collision. Particularly, hashing-based intersection can count triangles because hashing will put identical elements into the same bucket. However, with limited buckets, hashing will also put different elements into the same bucket, known as collisions. % searching through this gigantic hash table suffers from random access and lower cache hit~\cite{shun2015multicore}. 
\update{
To lower the collision cost,~\cite{shun2015multicore} allocates a gigantic memory space that is $l\times$ the original graph size. Afterwards, each vertex $u$ would take $l\times degree_u$ space from the gigantic memory space to build $u$'s hash table. Empirically, $l$ could be 2 - 4 if we want the cost of the collision to be low. Given this design needs a large memory region for hash table, ~\cite{shun2015multicore} observes high cache misses for their designs thus claims merge-path based method is better for triangle counting on CPUs. }
% proposes linear probing to manage collision, which saves some space from bitmap but ends up with non-trivial probing complexity.
% Tom et al.\cite{tom2017exploring} attempts to optimize this design by allocate thread count number of hash tables, which each of them to be 16$\times$ the maximum degree of the graph. This again suffers from large memory cost.
Later,~\cite{che2019accelerating,bisson2017high,bisson2018update}
% \update{~\cite{bisson2018update}}
% use as many buckets as the number of vertices (i.e., bitmap), ending up with overwhelming memory consumption and cache pressure. 
use bitmap to represent the hash bucket which still suffers from high cache pressure. 
% results in non-trivial design complexity that is hard to cope with all types of graphs. 
We also notice that \update{Yasar et al.~\cite{yacsar2018fast,yacsar2019linear,wolf2017fast,yasar2019linear,acer2019scalable}}
% \update{~\cite{yacsar2018fast}}
switch between dense and sparse representations of a hash table in their matrix multiplication effort which is, however, complex in nature. 

% in order to avoid collisions, mitigate space complexities, and alleviate probing penalty, which is, again, complex in nature. 
% \confuse{we describe Sivasankaran Rajamanickam method here}

In this paper, by reordering the graph, adjusting GPU hardware resources with respect to the vertex degree, we turn collision into a tolerable issue. 
% we find that collision is actually a tolerable issue on GPU if we can properly reorder the graph, use GPU thread hierarchy, and shared memory cache to combat the collision. 
Further, the potential of hashing is not fully unleashed, i.e., hashing can not only implement intersection, but also rapidly distribute workload across many-threads on GPUs, as well as graph partitions. 

% ing-based workload partition bests vertex-range based vertex and workload partition. 
% Second, collision is a tolerable issue on GPUs if we can properly reorder the graph, use GPU thread hierarchy and shared memory. 


% Hash table or bitmap require large memory, while GPU has limited global memory. And large hash table and bitmap will lead to low cache hit in querying.

\vspace{0.05in}
\textit{Challenge 2}. Vertex-centric triangle counting is worse than the edge-centric counterpart on GPUs due to worse workload imbalance issue~\cite{hu2018tricore,hu2017trix,hu2018high,pandey2019h}. 
% \update{~\cite{hu2018tricore}}. 
% The former one iterates through each vertex, fetches its 1-hop and 2-hop neighbor lists, and intersects these two neighbor lists in order to enumerate the triangles. The latter option iterates through each edge and counts the common neighbors from the source and destination vertices of the edge.}.
% \fixme{Add contents to support}
% Intuitively, vertex-centric is 
% Intuitively, vertex-centric method~{\cite{shun2015multicore,tom2017exploring,yacsar2018fast,yacsar2019linear,wolf2017fast,yasar2019linear,che2019accelerating}} counts triangles from a vertex perspective while edge-centric design~{\cite{hu2018tricore,hu2017trix,hu2018high,pandey2019h}} does so from edges.
Particularly, vertex-centric option~\cite{shun2015multicore,yacsar2018fast,yacsar2019linear,wolf2017fast,yasar2019linear,che2019accelerating} 
% \update{~\cite{shun2015multicore}}
iterates through each vertex, loads the 1- and 2- hop neighbors, and intersects them to arrive at the triangles. Edge-centric option~\cite{hu2018tricore,hu2017trix,hu2018high,pandey2019h}
% \update{~\cite{hu2018tricore}}
does that for each edge thus only 1-hop neighbors are needed. As a result, workload imbalance would arise from both inter- and intra- vertex aspects in vertex-centric design while the edge-centric counterpart only experiences workload imbalance across edges. 
%For the inter-vertex workload imbalance
Mathematically,
the time complexity of vertex-centric design is $\mathcal{O}(d(u)+\sum_{v\in N(u)}d(v))$ for vertex $u$ while that of edge-centric design is merely $\mathcal{O}(d(u)+d(v))$ between $u$ and $v$, where $d(u), d(v)$ and $N(u)$ are the degrees of $u$ and $v$, and the neighbor list of $u$, respectively. Hence, the workload difference between vertices is often higher than that of edges.
%\lld{Not clear which complexity is which one, edge-centric or vertex-centric.}
% So it's hard to balance the workload between different vertex and hard to get the workload of vertex. 
In terms of intra-vertex imbalance, 
% modern GPUs support massive thread in parallel. Use one thread process one vertex in not a good choice in GPU. It's easy to distribute task in edge centric, we only need to divide the intersection task. 
for each vertex $u$, we need to intersect $u$'s neighbor list with all its 2-hop neighbor lists, where the workloads of different 2-hop neighbor lists are also likely to be dissimilar. 
% the task is harder to distribute because we can't easy get the workload size and divide it.
% Edge-centric can achieve larger parallelism and better workload balance.
\update{Note, both vertex-centric and edge-centric algorithms perform accurate triangle counting and result in the same number of triangles}.

While the vertex-centric paradigm comes with the concern of imbalance, it also exhibits unique advantages. 
%{ This paradigm is popular in CPU based triangle counting systems~\cite{shun2015multicore,tom2017exploring,yacsar2018fast,wolf2017fast,che2019accelerating}.}
%\lld{Maybe move this sentence to somewhere else.}
First, the vertex-centric design avoids the need for edge list format, which saves $\frac{2}{3}$ of space and data movement traffic~\cite{hu2018tricore}. Second, for hashing-based intersection, the vertex-centric design largely reduces the cost of constructing the hash table compared to edge-centric method~\cite{pandey2019h}. Note, we find the innate GPU thread and memory hierarchy is a great remedy for workload imbalance. 

% \vspace{.1in}
% \fixme{Discuss workload first?}
\vspace{0.05in}
{\textit{Challenge 3}. The vertex-centric design makes distributed triangle counting a grand challenge stemming from the hardship of achieving communication free and workload balanced graph partitioning for vertex-centric triangle counting.}
% \fixme{Add contents to support}
As graphs continue to grow, a single machine (or device) will eventually fail to accommodate a large graph in memory. 
As a result, researchers rely upon either external memory options~\cite{kumar2016g,hu2013massive,chu2011triangle,pearce2013scaling}
% \update{~\cite{kumar2016g}}
or distributed settings~\cite{hu2017trix,hu2018tricore}
% \update{~\cite{hu2018tricore}}
to resolve this problem. 
% The former requires loading graph from external storage, which often takes longer time than in-memory method. For the latter solution, 
% in order to facilitate distributed in-memory triangle counting, we 
In order to achieve better performance, both designs will need communication free and workload balanced graph partitioning.
However, even for edge-centric design which only requires 1-hop neighbor lists, achieving both goals is challenging, which is evident both theoretically~\cite{hu2017trix,arifuzzaman2013patric} 
% \update{~\cite{hu2017trix}}
and practically~\cite{giechaskiel2015pdtl,hu2017trix,hu2018high,elenberg2015beyond,zhang2019litete}. 
% \update{~\cite{giechaskiel2015pdtl}}.
The vertex-centric design will require 2-hop neighbors, thus further exacerbates the problem. Particularly, 
towards communication free, one need to align the vertex ranges of 1-hop and 2-hop neighbors.
For the goal of workload balance, we will need similar 
$\mathcal{O}(d(u)+\sum_{v\in N(u)}d(v))$ across various partitions, where $u$ and $v$ are the vertices in one graph partition.

% estimate the workload of a vertex so that we can achieve similar workload across partitions.
% in vertex-centric triangle counting.
% The neighbor of vertex can be any vertex, and we require neighbor's neighbor. So it's hard to partition the graph. Imbalance between process each vertex is much larger than process edge in edge-centric. In partition, it's hard to estimate workload.

% \fixme{Corresponds to the third contribution}
In this work, we separate the goal of communication free and workload balance during graph partitioning. For the first goal, we propose a 2D graph partitioning that partitions the 1-hop neighbor and uses the 1-hop partitions to build the 2-hop ones. And we further partition the workload in order to scale {\hash} up to 1,000 GPUs. 
% In this context, the workload of each graph partition can be fulfilled by more than one combination of graph partitions. 
The workload balancing goal is achieved by hashing-based partitioning over our reordered graph.
% graph reordering and hashing. 

\begin{figure*}[t]
	\centering

	% \subfloat[neighbor list]
	% {
	% \includegraphics[width=3.8cm]{fig/intersection_a.pdf}
	% }
	% \subfloat[merge-path]{
	% \includegraphics[width=5cm]{fig/intersection_b.pdf}
	% }
	% \subfloat[binary-search]{
	% \includegraphics[width=3.5cm]{fig/intersection_c.pdf}
	% }
	% \subfloat[hash]{
	% \includegraphics[width=4cm]{fig/intersection_d.pdf}
	% }
	\includegraphics[width=.9\textwidth]{fig/intersection.pdf}

	\caption{Five triangle counting methods. (a) M and N are the neighbor lists used by (b) - (d) which are merge-path, binary-search, and hashing-based intersection.  
% 	\vspace{-0.1in}
	}
	\label{intersection}
	\vspace{-.25in}
\end{figure*}
\vspace{-0.05in}
\subsection{Contributions}
This paper designs and implements a vertex-centric hashing-based triangle counting system on GPUs that can achieve beyond 1 trillion TEPS performance on random, rMat, and 3Dgrid graphs.  
Particularly, this work not only reveals and leverages the unique advantages of hashing and vertex-centric options for scalable triangle counting on GPUs but also carefully designs optimizations to overcome the key challenges faced by the vertex-centric hashing method. 
In summary, this work makes the following contributions. 


% \vspace{0.05in}
First, vertex-centric hashing presents great potentials for GPU-based triangle counting. 
% \fixme{Add contents to support}
In spite of collision concern, hashing-based intersection exhibits advantageous features over both merge-path~\cite{green2014fast} and binary-search~\cite{hu2018tricore} based counterparts~\cite{DBLP:conf/alenex/2014,DBLP:conf/alenex/OrtmannB14}.
% \update{~\cite{DBLP:conf/alenex/OrtmannB14}}.
Particularly, merge-path suffers from workload partitioning hardship, while hashing does not. Binary-search experiences high time complexity \update{i.e. $\mathcal{O}(logN)$}, and hashing lowers that cost to \update{i.e. $\mathcal{O}(1)$}. \update{Furthermore, binary-search requires random access to the data stored in a binary tree, which will experience uncoalesced memory access.} 
Similarly, for vertex- vs. edge- centric paradigms: while the edge-centric option requires both edge list and adjacency list of a graph, the vertex-centric option only needs the latter. 
Putting hashing and vertex-centric paradigms together, {\hash} avoids repeated hash table construction in edge-centric design~\cite{pandey2019h}.
On average, the vertex-centric option reduces the hash table construction time by 92$\times$.
When deployed on GPUs, we interleave the entries from all buckets and exploit GPU shared memory to lower the hash table lookup cost. 

% subsequently use GPU shared memory to lower the {collision cost}. Note, we also interleave the entries of all the buckets to coalesce memory accesses.
% \confuse{in global memory}.

% 1) Hash table construction is a costly operation in edge-centric. Vertex-centric delete the duplicate hash table construction for same vertex. 2) we use the hash table that allow collision to achieve better memory access.

% \vspace{0.05in}
Second, admittedly, vertex-centric hashing also comes with drawbacks, i.e., collision and workload imbalance, which requires optimizations. 
% \fixme{Add contents to support}
Towards collision reduction, we propose a graph reordering technique that reorders the vertex IDs of a graph.
%\lld{Didn't introduce what is reordering, so it's hard to make sense of the rest of the paragraph.}
% Though optimal reordering is complex
% \confuse{should we notice that we prove its NP hard?} 
% in nature~\cite{han2018speeding,wei2016speedup}, 
Since optimal reordering is NP-complete, we find two effective heuristics. The intuition behind these heuristics is that we should give priority to high-degree vertices and their neighbors when lowering the collisions. This approach enhances performance by {up to 75\%}. For intra-vertex workload imbalance, we introduce a virtual combination to virtually combine the 2-hop neighbors together in order to ultimately balance the intra-vertex workload. This yields, on average {50\%} speedup across graphs. Taken collision and inter-vertex workload imbalance together, we exploit degree-aware resource and thread assignment mechanisms that give large degree vertices more hash buckets, shared memory, and threads. This design yields, on average, {7$\times$} speedup across all the graphs. 
% \confuse{Further our atomic load vertex achieve 20$\%$ speedup.}



% \vspace{0.05in}
% \fixme{reword}
Third, we introduce workload and graph collaborative, and hashing-based 2D partitioning scheme to scale triangle counting beyond 1,000 GPUs. 
% \fixme{Add contents to support}
Particularly, we use hashing, instead of vertex range, to partition the graph into 2D (i.e., partition both source and destination vertices) so that each partition comes with a similar workload, thanks to our graph reordering method. 
% \lld{what is 2D?}
% \confuse{we can show the IR(min GPU time/max GPU time) of large graph}. 
Subsequently, for each 1-hop neighbor partition that is used for hash table construction, we use the 1-hop neighbor partitions to build up the 2-hop neighbor partitions because our 2D partition ensures the source and destination vertices are evenly partitioned. The partitioning approach is detailed in Figure~\ref{fig:Graph partition}(b). 
% That is,  we use all the out neighbor partitions to extract the 2-hop neighbor
% several 2-hop neighbor partitions are needed to count the triangles. 
Since different 2-hop partitions can enumerate the triangles independently,
% After each graph partition can fit in GPU memory, 
we further introduce workload partitioning, which distributes various 2-hop neighbor partitions across more GPUs. Taken together, our graph and workload collaborative partitioning can saturate 1,024 GPUs with merely 64 graph partitions.
This design is not only space and workload balanced but also communication free. Particularly, for extremely large graphs, we achieve 1.9$\times$ speedup from 512 to 1,024 GPUs and beyond 600$\times$ speedup for medium graphs from 1 to 1,024 GPUs. 
\vspace{-0.2in}
% and achieve linear scalability in large graph.
% To balance workload between subtasks, we use hash to partition graph and workload. Due to the reordering and degree aware resource assignment, hash based partition achieve good balance between subtasks.
% 1) we propose workload partition to scale \hash to multi GPU and graph partition to scale \hash to large graph. Further, we combine these two method together to achieve better scalability. 2) we use hash to partition graph and workload which achieve better balance.
\subsection{Paper Organization}
The rest of this paper is organized as follows. Section~\ref{sec:background} presents the background. 
% Section~\ref{sec:related} presents some related works in triangle counting and conventional triangle counting algorithms. 
Section~\ref{sec:hash} describes the novel {\hash} designs. 
Section~\ref{sec:opt} presents the optimization techniques for hash collision and workload imbalance.
Section~\ref{sec:scale} presents our workload and graph collaborative partition methods.
Section~\ref{sec:eval} evaluates the performance of {\hash} and Section~\ref{sec:conclusion} concludes.



% Triangle counting can be formulated into problems from two different domains, that is, graph computing and graph mining.
% % Mainstream triangle counting algorithms mainly consists of efforts in two directions, graph computing and mining. 
% The former domain further encompasses vertex and edge-centric approaches~\cite{latapy2008main}. The vertex-centric one iterates through each vertex, fetches its neighbors, and counts the pair of neighbors that possess intermediate edge(s), while \textbf{the edge-centric option iterates through each edge and counts the common neighbors from the source and destination vertices of the edge}. In graph mining domain, one will first find all open triangles through tree-based prune and subsequently verify whether there exists an edge from the graph that can complete this triangle~\cite{bhattarai2019ceci}. 

% Given edge-centric approach outperforms the other alternatives~\cite{hu2018tricore,hu2018high,shun2015multicore}, intersecting two sorted neighbor lists to count the common ones becomes the key for triangle counting. Particularly, there are two mainstream designs on this track, that is, merge-path and binary-search based methods. Assuming two neighbor lists - $M$ and $N$ - are at size of $|M|$ and $|N|$, where $|M|\le |N|$, the time complexities of merge-path and binary-search based designs are $\mathcal{O}(|M|+|N|)$~\cite{giechaskiel2015pdtl,green2014fast} and $\mathcal{O}(|M|\cdot log|N|)$~\cite{hu2018tricore}, respectively. Therefore, binary-search based approach is deemed more efficient when $|M|>>|N|$. However, the popular edge orientation method~\cite{hu2017trix} will shrink the difference between $M$ and $N$ drastically, leading merge-path to be more efficient, in terms of time complexity, than binary-search based alternative. Surprisingly, TriCore~\cite{hu2018tricore} demonstrates that binary-search based design is significantly faster than the merge-path based one, blaming the hardship of properly distributing the workload across GPU threads and the unfriendly memory access patterns of merge-path based approach. 
% % But, the performance of TriCore~\cite{hu2018tricore} depends heavily upon the size of the neighbor list. The algorithmic complexity of binary search is disadvantageous. 

% % Intersection based approaches are assumed to have state of the art performance in triangle counting with GPUs.~\cite{shun2015multicore} empirically states that intersection based approaches yield better performance than other approaches. Although merge based intersection have less complexity than binary search intersection, it is not much flexible for parallelization over GPU and needs both lists to be sorted.~\cite{green2014fast} implements parallel merge based intersection adopting partitioning neighbor list into disjoint sets so that each thread could work on each disjoint set. It uses binary search to create disjoint sets which incur extra overhead for each edge. Also, during partitioning, it suffers from strided memory access pattern. Tricore~\cite{hu2018tricore} proposes a binary search based intersection suggesting to have better performance as it would only require to sort a single list and another is used as lookup. Further, they cache some level of search tree for better memory access. 





% For the completeness of related work review, we also briefly discuss other approaches. For instance, subgraph matching  based design~\cite{wang2016comparative} and matrix multiplication based design~\cite{Yasar2018FastTC} are also found in some related work, but requires more memory or performs unavoidable redundant work~\cite{wang2016comparative}.~\cite{bisson2017high} implements bitmap based intersection but requires atomic operations to update the bitmap in parallel and also suffers from strided memory access pattern. Hashing have the best algorithmic complexity for lookup compared to other.


% % ~\cite{shun2015multicore} implements hash based method for TC designed for multi-core machines but would not be able to perform well on GPUs. Overcoming these hindrance, we design a GPU friendly and scalable hash based approach for Triangle counting.

% This work proposes {\hash}, a hash-indexing based approach to accelerate parallel triangle counting. 
% % Particularly, we propose three hash-related algorithms, that is, {\hash} standalone approach, and {\hash} accelerated merge-path and binary-search based designs. Eventually, we evaluate the proposed the three {\hash} related algorithms atop various GPUs and demonstrate the superior performance over the state-of-the-art efforts. This achievement is not possible without the following contributions.

% First, inspired by the observation that only items that experience collision will have the chance of being intersected, we use hash to distribute the workload. Basically, {\hash} first conducts hash on the shorter neighbor list (i.e., $N$) partition various entries into different buckets, hoping shorter neighbor list will experience lower chance of hashing different neighbor lists to the same bucket. Afterwards, {\hash} iterates through the longer list (i.e., $N$), and conducts hash again. This time, {\hash} first hash each neighbor into a corresponding bucket, then finds whether there is a common neighbor in that bucket from the shorter list. If the corresponding bucket contains more than one value, a linear-search will be performed. 

% Second, to coalesce the memory access, we interleave hash entries from various hash buckets for the shorter neighbor list. That is, the first element of all buckets are stored consecutively, subsequently the second element and etc. This design stems from the fact that, during searching for common neighbors, all threads (of a Warp or CTA) will start from the first element in various buckets. Storing all the elements from the same bucket adjacently will introduce strided memory access. 


% Merge-path based approach consists of three weakness: 1) hard to partition. \cite{Green,green2014fast} using binary-search to partition neighbor list. However, it has imbalance workload and need non-trivial cost. 2) stride in memory access. For example, we partition $N(1)$ into two list using binary-search. One thread will scan the list from top to mid while another scan the list from mid to end. 3) neighbor list need to be sorted in preprocessing, which introduce cost.
 
% Binary-search based option 1) high time complexity. When $d(v)$ and $d(u)$ is close time complexity is relatively high. When $d(v)=d(u)=64$, we need $64*\log_2 64=384$ operations. Hash based triangle counting only needs 64 operations in intersection when the $HT_u$ has been construct and has no collision. 2) stride in memory access. For example, we have two thread to process $5, 7$ in $N(1)$, it has stride access in the second level of binary-search when search $4, 8$ and in the third level when search $5, 7$.   3) neighbor list need to be sorted in preprocessing.
  
 
% Bitmap has much lower time complexity but has a big problem. It requires large memory space for each vertex. Or we can dynamic construct the bitmap from neighbor list, but the initial of bitmap cost O($|V|$). And there still have stride memory access in bitmap query. Furthermore, we can transform hash to bitmap as discussed before.






% % For binary-search approach, it will also hash both $M$ and $N$ into 32 buckets. However, it only need one neighbor list to be sorted. Potentially, this reduces the partitioning overhead comparing to {\hash} assisted merge-path alternative.
% It is also important to note that {\hash} avoids sorting the neighbor lists during preprocessing, which is essential and time consuming for both binary-search and merge-path based approaches.

% % Second, we propose {\hash} assisted merge-path and binary-search designs. For merge-path approach, {\hash} first uses hash to partition both neighbor lists into 32 buckets. Note, this approach involves exclusive prefix-sum to arrive at sorted entries in each bucket for both $M$ and $N$. Afterwards, each thread will be responsible for one bucket of sublists from both $M$ and $N$. Note, to coalesce the memory access from a warp of threads, we interleave the items 32 buckets. For binary-search approach, it will also hash both $M$ and $N$ into 32 buckets. However, it only need one neighbor list to be sorted. Potentially, this reduces the partitioning overhead comparing to {\hash} assisted merge-path alternative.

% \textbf{Highlights}. Despite we avoid the tremendous preprocessing overhead on the graph datasets comparing to all existing work, 
% {\hash} still manages to achieve $10^{9}$ TEPS for a large portion of the graph challenge datasets. Most importantly, {\hash} retains a maximum of 40.169 billion TEPS on the MAWI-e38040320 graph. {Note, without the preprocessing (sorting the neighbor list), all proposed triangle counting algorithms will fail to work.}


% Brief History of Triangle Counting

% List Merging and Triangle Counting

% Merge based approaches and binary search approaches

% Why merge based methods are slow in GPU?

% Contributions of this paper: How we make merge faster?

% Overview of the Paper

==> related-work.tex <==
\section{Other related Work}
% \subsection{Exact Triangle Counting}
% Reviewing the recent literature centering around triangle counting~\update{\cite{shun2015multicore,che2019accelerating,bisson2017high,bisson2018update,yacsar2018fast,yacsar2019linear,wolf2017fast,hu2017trix,hu2018tricore,hu2018high,hu2019triangle,chu2011triangle,date2017collaborative,pearce2017triangle,elenberg2015beyond,arifuzzaman2015fast,tom20192d,tom2017exploring,hoang2019disttc,pandey2019h,hu2013massive,giechaskiel2015pdtl,cui2018efficient,yasar2019linear,zhang2019litete,green2014fast,azad2015parallel,Low2017FirstLL,acer2019scalable,wang2016comparative,bisson2017static,DBLP:conf/alenex/2014,DBLP:conf/alenex/OrtmannB14}}, we arrive at the following pitfalls, along with our proposed resolutions.  
% % - {edge-centric list intersection is the most popular option for triangle counting}. In terms of intersection algorithms, merge-path excels on CPU while binary-search bests on GPU. When it comes to distributed triangle counting, edge-centric again prevails. We explain the key reasons behind these pitfalls and our resolutions as below: 


% % have explored the possibility of applying hashing to aid triangle counting, they fall short at fully unleash the potential of hashing.


% {Pitfall 1. Hash-based intersection is not suitable for triangle counting} resulting from the concern of collision. Particularly, we leverage the nature of hash, which puts the identical elements into the same bucket, to count triangles. However, with limited buckets, hash will also put different elements into the same bucket, known as collision. In order to address this concern,~\cite{che2019accelerating,bisson2017high,bisson2018update} use as many buckets as the number of vertices (i.e., bitmap), ending up with overwhelming memory consumption. 
% % searching through this gigantic hash table suffers from random access and lower cache hit~\cite{shun2015multicore}. 
% Alternatively,~\cite{shun2015multicore} proposes linear probing to manage collision, which strives to save some space from bitmap but ends up with non-trivial probing complexity. 
% % results in non-trivial design complexity that is hard to cope with all types of graphs. 
% We also notice that~\cite{yacsar2018fast,yacsar2019linear,wolf2017fast,yasar2019linear} switch between dense and sparse representations of a hash table in order to avoid collisions, mitigate space complexities and alleviate probing penalty, which is, again, complex in nature. 
% % \confuse{we describe Sivasankaran Rajamanickam method here}

% By reordering the graph, utilizing GPU thread hierarchy, and shared memory cache, we not only combat collisions, but turn them into a tolerable issue. 
% % we find that collision is actually a tolerable issue on GPU if we can properly reorder the graph, use GPU thread hierarchy and shared memory cache to combat the collision. 
% Further, the potential of hashing is not fully unleashed, i.e., hash can not only implement intersection, but also rapidly distribute workload across many-threads on GPUs. 

% % ing-based workload partition bests vertex-range based vertex and workload partition. 
% % Second, collision is a tolerable issue on GPUs if we can properly reorder the graph, use GPU thread hierarchy and shared memory. 


% % Hash table or bitmap require large memory, while GPU has limited global memory. And large hash table and bitmap will lead to low cache hit in querying.


% {Pitfall 2. Vertex-centric triangle counting performs worse than the edge-centric counterpart \update{when implemented on GPU}.}
% % \fixme{Add contents to support}
% % Intuitively, vertex-centric is 
% Intuitively, vertex-centric method~\update{\cite{shun2015multicore,tom2017exploring,yacsar2018fast,yacsar2019linear,wolf2017fast,yasar2019linear,che2019accelerating}} counts triangles from a vertex perspective while edge-centric method~\update{\cite{hu2018tricore,hu2017trix,hu2018high,pandey2019h}} from an edge. Thus, vertex-centric option iterates through each vertex, loads the 1- and 2- hop neighbors and intersects them to arrive at the triangles. Edge-centric does that for each edge thus only 1-hop neighbors are needed. In this way, the biggest concern of vertex-centric design is workload imbalance, including both inter- and intra- vertex aspects. 
% For the inter-vertex workload imbalance, the time complexity of a vertex $u$ is $\mathcal{O}(d(u)+\sum_{v\in N(u)}d(v))$ while that of an edge in edge-centric design is merely $\mathcal{O}(d(u)+d(v))$ between $u$ and $v$, where $d(u), d(v)$ and $N(u)$ are the degrees of $u$ and $v$, and the neighor list of u, respectively. Hence, the workload difference between vertices is often higher than that of edges. 
% % So it's hard to balance the workload between different vertex and hard to get the workload of vertex. 
% In terms of intra-vertex imbalance, 
% % modern GPUs support massive thread in parallel. Use one thread process one vertex in not a good choice in GPU. It's easy to distribute task in edge centric, we only need to divide the intersection task. 
% for each vertex $u$, we need to intersect $u$'s neighbor list with all its 2-hop neighbor list, where the workload of different 2-hop neighbor lists are also likely to be dissimilar. 
% % the task is harder to distribute because we can't easy get the workload size and divide it.

% % Edge-centric can achieve larger parallelism and better workload balance.

% While vertex-centric paradigm comes with the concern of imbalance, it also exhibits unique advantages. First, vertex-centric design avoids the need of edge list format which saves $\frac{2}{3}$ of the space and data movement traffic~\cite{hu2018tricore}. Second, for hash-based intersection, vertex-centric design largely reduces the cost of constructing the hash table compared to edge-centric method~\update{\cite{pandey2019h}}. \update{Vertex-centric is mostly popular in CPU based triangle counting systems~\cite{shun2015multicore,tom2017exploring,yacsar2018fast,wolf2017fast,che2019accelerating}}. Note, we find GPU thread and memory hierarchy is a great remedy for workload imbalance. 

% {Pitfall 3. Vertex-centric design, which requires 2-hop neighbor lists, is a grand challenge for graph partitioning.}
% % {Communication free, workload balanced partition for vertex-centric triangle counting is hard.}
% % \fixme{Add contents to support}
% As graphs continue to grow, single machine (or device) will eventually fail to count the triangle for a large graph in memory. As a result, researchers either explore external memory options~\cite{kumar2016g,hu2013massive,chu2011triangle,pearce2013scaling} or distributed settings to resolve this problem. 
% The former requires loading graph from external storage, which often takes longer time than in-memory method. 
% However, in order to facilitate distributed in-memory triangle counting, we need to partition the graph so that communication is minimal and workload is balanced. Even for edge-centric design which only requires 1-hop neighbor lists, this goal is challenging, both theoretically~\cite{hu2017trix,arifuzzaman2013patric} and practically~\cite{giechaskiel2015pdtl,hu2017trix,hu2018high,elenberg2015beyond,zhang2019litete}. 
% When it goes to vertex-centric design which requires 2-hop neighbors, the problem becomes even harder. Particularly, 
% % Some systems require communication between different nodes, which also slower the system efficiency.
% % The best choice is communication free distributed system. But partition graph in vertex centric to achieve communication free is hard. 
% first, the neighbors of a vertex are random,
% % if one processor need to process this one vertex it needs to load whole graph, And we also need 
% the requirement of 2-hop neighbor lists further adds the complexity for communication-free partition. Further, it is hard to partition the graph so that the 2-hop neighbor associated workload is roughly balanced. 
% % estimate the workload of a vertex so that we can achieve similar workload across partitions.
% % in vertex-centric triangle counting.
% % The neighbor of vertex can be any vertex, and we require neighbor's neighbor. So it's hard to partition the graph. Imbalance between process each vertex is much larger than process edge in edge-centric. In partition, it's hard to estimate workload.

% In this work, we showcase that partitioning a graph for vertex-centric implementation is actually analogous to edge-centric after we separate the partitioning of graph data and workload. 
% %  we introduce a workload and graph collaborative partitioning method that detaches the partition of the 1-hop and 2-hop neighbor lists. 
% In this context, the workload of each graph partition can be fulfilled by more than one combination of graph partitions. The workload balancing is achieved by hashing based partitioning on our reordered graph.
% % graph reordering and hashing. 



